From Operational Design Domain to Action: A Systematic Behavioral Taxonomy for Autonomous Driving

Operational Design Domain (ODD) specifications describe where an automated driving system (ADS) is permitted to operate, but they do not prescribe what the ADS must demonstrably do once deployed within that domain. This gap between operating condition specification and behavioral validation represents a critical unresolved challenge in ADS safety assurance. This paper presents a structured, standards-grounded taxonomy of 21 behavioral competencies organized across three operational domains-Highway (HWY), Urban (URB), and Hub (HUB)-derived systematically from the PEGASUS six-layer model-based ODD. Each behavior is decomposed along longitudinal and lateral control axes and characterized against a four-property framework: Safety (gap maintenance, conflict avoidance, kinematic stability), Compliance (legal rules and behavioral norms), Comfort (rider dynamics and trust), and Efficiency (mission completion and product-level metrics). We further demonstrate that the crossing of ODD layer parameterizations with behavioral competency specifications yields concrete scenario families suitable for systematic behavioral testing and SOTIF coverage evidence. The taxonomy is grounded in AVSC00008202111, SAE J3237, and SAE J3016, and is validated as an operational specification layer through its deployment in a rule-enforced trajectory optimization system. The Hub domain is identified as a structurally distinct, underspecified domain warranting dedicated research attention.

==> figures/fig_odd_gap.tex <==
% figures/fig_odd_gap.tex
% ODD → ??? → Validation gap diagram — NOT CURRENTLY USED IN TEXT
% (kept as optional figure; add \input{figures/fig_odd_gap.tex} to
%  Introduction if space permits)

\begin{tikzpicture}[
  box/.style={
    rectangle, rounded corners=4pt,
    minimum width=2.4cm, minimum height=2.8cm,
    draw, line width=0.7pt,
    font=\scriptsize, align=center, inner sep=4pt
  },
  arr/.style={-{Stealth[length=5pt]}, thick, dashed}
]

% ODD box
\node[box, fill=blue!10, draw=blue!50!black] (odd) at (0,0) {
  \textbf{ODD}\\[4pt]
  \tiny
  PEGASUS\\
  6-Layer Model\\[4pt]
  Defines\\
  \emph{WHERE}
};

% Gap
\node[font=\huge\bfseries, text=red!70] (q) at (2.9,0) {?};
\draw[arr, color=red!60] (1.3,0) -- (2.3,0);
\draw[arr, color=red!60] (3.5,0) -- (4.5,0);
\node[font=\tiny\itshape, text=red!60, align=center]
  at (2.9,-1.6) {No behavioral\\specification layer};

% Validation box
\node[box, fill=red!5, draw=red!40] (val) at (5.8,0) {
  \textbf{ADS}\\
  \textbf{Validation}\\[4pt]
  \tiny
  Scenario suites\\
  SOTIF evidence\\[4pt]
  Requires\\
  \emph{WHAT}
};

% Bridge label below
\node[font=\scriptsize\bfseries, text=navyblue,
      draw=navyblue!30, rounded corners=2pt,
      fill=blue!5, inner sep=3pt]
  at (2.9,-2.5) {Behavioral Competency Taxonomy fills this gap};

\draw[-{Stealth[length=4pt]}, navyblue!60, dashed]
  (2.9,-2.1) -- (2.9,-0.6);

\end{tikzpicture}


==> figures/fig_taxonomy.tex <==
% figures/fig_taxonomy.tex
% Domain taxonomy overview — three cards with Lon/Lat/Both bars

\begin{tikzpicture}[
  domcard/.style={
    rectangle, rounded corners=4pt,
    minimum width=2.2cm, minimum height=4.8cm,
    draw, line width=0.6pt
  },
  hdr/.style={
    rectangle, rounded corners=3pt,
    minimum width=2.0cm, minimum height=0.55cm,
    font=\footnotesize\bfseries, text=white,
    align=center
  },
  axlabel/.style={font=\scriptsize\bfseries},
  axbar/.style={rectangle, rounded corners=2pt, minimum height=0.3cm}
]

% ── HWY card ──────────────────────────────────────────────────
\node[domcard, fill=blue!5, draw=blue!40] (hwy) at (0,0) {};
\node[hdr, fill=blue!70!black] at (0, 1.9) {HWY};
\node[font=\scriptsize, text=blue!70!black] at (0, 1.35) {8 behaviors};

% Lon bar (3/8)
\node[axlabel, text=blue!80!black] at (-0.3, 0.85) {Lon};
\node[axbar, fill=blue!70, minimum width=1.5cm] at (0.45, 0.85) {};
\node[font=\scriptsize, text=white] at (0.45, 0.85) {3};

% Lat bar (2/8)
\node[axlabel, text=blue!80!black] at (-0.3, 0.35) {Lat};
\node[axbar, fill=blue!50, minimum width=1.0cm] at (0.35, 0.35) {};
\node[font=\scriptsize, text=white] at (0.35, 0.35) {2};

% Both bar (3/8)
\node[axlabel, text=blue!80!black] at (-0.3,-0.15) {Both};
\node[axbar, fill=blue!90!black, minimum width=1.5cm] at (0.45,-0.15) {};
\node[font=\scriptsize, text=white] at (0.45,-0.15) {3};

\node[font=\tiny\itshape, text=gray, text width=2.0cm, align=center]
  at (0,-1.0) {High-speed\\Structured lanes\\Vehicle-dominant};

% ── URB card ──────────────────────────────────────────────────
\node[domcard, fill=green!5, draw=green!50!black!40] (urb) at (2.7,0) {};
\node[hdr, fill=green!50!black] at (2.7, 1.9) {URB};
\node[font=\scriptsize, text=green!50!black] at (2.7, 1.35) {8 behaviors};

\node[axlabel, text=green!60!black] at (2.4, 0.85) {Lon};
\node[axbar, fill=green!60!black, minimum width=2.0cm] at (3.05, 0.85) {};
\node[font=\scriptsize, text=white] at (3.05, 0.85) {4};

\node[axlabel, text=green!60!black] at (2.4, 0.35) {Lat};
\node[axbar, fill=green!40!black, minimum width=1.0cm] at (2.95, 0.35) {};
\node[font=\scriptsize, text=white] at (2.95, 0.35) {2};

\node[axlabel, text=green!60!black] at (2.4,-0.15) {Both};
\node[axbar, fill=green!70!black, minimum width=1.0cm] at (2.95,-0.15) {};
\node[font=\scriptsize, text=white] at (2.95,-0.15) {2};

\node[font=\tiny\itshape, text=gray, text width=2.0cm, align=center]
  at (2.7,-1.0) {Mixed agents\\Intersections, VRUs\\Traffic signals};

% ── HUB card ──────────────────────────────────────────────────
\node[domcard, fill=orange!5, draw=orange!60!black!40] (hub) at (5.4,0) {};
\node[hdr, fill=orange!70!black] at (5.4, 1.9) {HUB};
\node[font=\scriptsize, text=orange!70!black] at (5.4, 1.35) {5 behaviors};

\node[axlabel, text=orange!70!black] at (5.1, 0.85) {Lon};
\node[axbar, fill=orange!60!black, minimum width=1.0cm] at (5.75, 0.85) {};
\node[font=\scriptsize, text=white] at (5.75, 0.85) {2};

\node[axlabel, text=orange!70!black] at (5.1, 0.35) {Lat};
\node[axbar, fill=orange!40!black, minimum width=1.0cm] at (5.75, 0.35) {};
\node[font=\scriptsize, text=white] at (5.75, 0.35) {2};

\node[axlabel, text=orange!70!black] at (5.1,-0.15) {Both};
\node[axbar, fill=orange!80!black, minimum width=0.5cm] at (5.55,-0.15) {};
\node[font=\scriptsize, text=white] at (5.55,-0.15) {1};

\node[font=\tiny\itshape, text=gray, text width=2.0cm, align=center]
  at (5.4,-1.0) {Geofenced facility\\DDT-F heavy\\Internal ruleset};

% Total label
\node[font=\scriptsize\bfseries, text=navyblue]
  at (2.7,-2.55) {21 Behavioral Competencies across 3 ODD-Derived Domains};

\end{tikzpicture}

